Safety Screening for Voltage Control in Active Distribution Grids via Distributionally Robust Conformal Screening

Deploying a new control policy for voltage control in active distribution grids requires evidence that physical limits will be satisfied before the policy is tested on the physical grid. This assessment is difficult for two reasons. First, simulations cannot capture every disturbance, modeling error, and device interaction present in the real grid. Second, historical measurements reflect operation under existing control policies, whereas a new policy may drive the grid into different operating conditions. To address these challenges, we propose Distributionally Robust Conformal Safety Screening (DR-CSS), a policy-agnostic framework for pre-deployment, scenario-by-scenario screening of a new control policy using historical data and a nominal simulator. For each new scenario, the simulator predicts a future voltage trajectory for the whole grid; DR-CSS then constructs a conformal safety interval around this prediction using historical simulation-to-reality errors. The interval is further enlarged to account for closed-loop changes induced by the deployment of the new policy and its interactions with the remaining controllers. To the best of our knowledge, DR-CSS is the first framework in power systems to combine historical data from an existing control policy with an imperfect simulator for pre-deployment safety screening of a new policy. Experiments on the IEEE 33-bus and IEEE 141-bus systems evaluate the deployment of learning-based voltage control policies and show that DR-CSS identifies all unsafe test scenarios. To reduce unnecessary warnings on safe scenarios, we adapt the safety intervals to different operating conditions and gradually introduce new policies with recalibration after each stage. These extensions increase the informational value of the safety screening and support safer deployment decisions in active distribution grids.

==> 02_related_work_table.tex <==

\begin{table*}[t]
\centering
\caption{Positioning of DR-CSL relative to related assurance approaches.
\(\checkmark\) = central to the method;
\(\triangle\) = partially addressed or requires additional assumptions;
\(--\) = not the main focus.}
\label{tab:positioning}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{p{0.27\textwidth}ccccc}
\toprule
\multirow{2}{*}{Approach}
  & Feeder        & Coverage      & Robust to     & Learned-policy & Operational \\
  & voltage control  & guarantee     & dist.\ shift  & validation     & scenario flag \\
\midrule
%──────────────────────────────────────────────────────────────────
% Row 1 – simulation / hardware-in-the-loop
Scenario simulation / HIL
\cite{Wang2019PHIL,OTT18,PAS24}
  & \(\checkmark\) & \(-\!\,-\)    & \(-\!\,-\)    & \(\triangle\)  & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 2 – set-based / symbolic formal verification
Formal verification / reachability
\cite{Tran2022VerificationLECPS,%
      Everett2021NNVerification,Kochdumper2023OpenClosedLoop}
  & \(\triangle\)  & \(\triangle\) & \(-\!\,-\)    & \(\triangle\)  & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 3 – constrained / safe RL for Volt-Var
Safe RL for Volt--Var control
\cite{Wang2020SafeOffPolicy,Gao2022ModelAugmentedSafeRL,%
      Nguyen2022OnlineSafeDRL,CUI2022108609}
  & \(\checkmark\) & \(-\!\,-\)    & \(-\!\,-\)    & \(\checkmark\) & \(-\!\,-\)    \\
%──────────────────────────────────────────────────────────────────
% Row 4 – standard CP + power-systems CP forecasting
Standard CP / CP in energy applications
\cite{VOV22,ANG22,LEI17,REN24,Renkema2024PVForecast,%
      FAU24,MOR25cacp,MAR25voltraj}
  & \(\triangle\)  & \(\checkmark\) & \(-\!\,-\)   & \(-\!\,-\)     & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 5 – CP under shift / off-policy CP
CP beyond exchangeability / off-policy CP
\cite{TIB20,BAR23,TAU22,KUI24}
  & \(-\!\,-\)     & \(\checkmark\) & \(\triangle\) & \(\triangle\)  & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 6 – CP for safety verification & control (autonomous systems)
CP for safety verification \& control
\cite{LIN24survey,ZHA23stl,CHE25ncbf,ZHA24cpp}
  & \(-\!\,-\)     & \(\checkmark\) & \(\triangle\) & \(\checkmark\) & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 7 – distributionally robust conformal validation
Robust conformal validation
\cite{CAU24,AOL25}
  & \(-\!\,-\)     & \(\checkmark\) & \(\checkmark\) & \(-\!\,-\)    & \(\triangle\) \\
%──────────────────────────────────────────────────────────────────
% Row 8 – this paper
\textbf{DR-CSL (this paper)}
  & \(\checkmark\) & \(\checkmark\) & \(\checkmark\) & \(\checkmark\) & \(\checkmark\) \\
\bottomrule
\end{tabular}
\end{table*}

==> figures/ablation_study/loadwise_rho_grid.tex <==
% Data files expected in \gridpath:
%   loadwise_rho_grid_uniform.csv
%   loadwise_rho_grid_specific.csv
%   loadwise_rho_grid_meta.csv
%
% Required in the main document preamble:
% \usepackage{pgfplots}
% \usepgfplotslibrary{groupplots}
% \usetikzlibrary{calc,patterns,plotmarks}
% \pgfplotsset{compat=1.18}

\providecommand{\gridpath}{figures/ablation_study/}
\providecommand{\loadbin}{4}

\definecolor{rwthred100}{HTML}{CC071E}
\definecolor{gridline}{HTML}{666666}

\newcommand{\drawpvpanelmark}[1]{
    \pgfscope
    % Conventional monochrome PV-panel symbol with support.
    \pgfsetstrokecolor{black}
    \pgfsetlinewidth{0.24pt}
    \pgfpathmoveto{\pgfpoint{0pt}{-.15\pgfplotmarksize}}
    \pgfpathlineto{\pgfpoint{0pt}{-.72\pgfplotmarksize}}
    \pgfpathmoveto{\pgfpoint{-.45\pgfplotmarksize}{-.72\pgfplotmarksize}}
    \pgfpathlineto{\pgfpoint{.45\pgfplotmarksize}{-.72\pgfplotmarksize}}
    \pgfusepathqstroke

    \pgfsetfillcolor{white}
    \pgfsetstrokecolor{#1}
    \pgfsetlinewidth{0.55pt}
    \pgfpathrectangle
        {\pgfpoint{-\pgfplotmarksize}{-.15\pgfplotmarksize}}
        {\pgfpoint{2\pgfplotmarksize}{1.0\pgfplotmarksize}}
    \pgfusepathqfillstroke

    \pgfsetstrokecolor{black}
    \pgfsetlinewidth{0.2pt}
    \pgfpathmoveto{\pgfpoint{-.34\pgfplotmarksize}{-.15\pgfplotmarksize}}
    \pgfpathlineto{\pgfpoint{-.34\pgfplotmarksize}{.85\pgfplotmarksize}}
    \pgfpathmoveto{\pgfpoint{.34\pgfplotmarksize}{-.15\pgfplotmarksize}}
    \pgfpathlineto{\pgfpoint{.34\pgfplotmarksize}{.85\pgfplotmarksize}}
    \pgfpathmoveto{\pgfpoint{-\pgfplotmarksize}{.35\pgfplotmarksize}}
    \pgfpathlineto{\pgfpoint{\pgfplotmarksize}{.35\pgfplotmarksize}}
    \pgfusepathqstroke
    \endpgfscope
}

\pgfdeclareplotmark{pvpanel}{\drawpvpanelmark{black}}
\pgfdeclareplotmark{pvpanelalert}{\drawpvpanelmark{rwthred100}}

\pgfplotsset{
    colormap={widthmap}{
        rgb255=(255,255,217);
        rgb255=(199,233,180);
        rgb255=(127,205,187);
        rgb255=(65,182,196);
        rgb255=(29,145,192);
        rgb255=(34,94,168);
        rgb255=(12,44,132)
    },
}

\pgfplotstableread[col sep=comma]{\gridpath/loadwise_rho_grid_meta.csv}\gridmeta
\pgfplotstablegetelem{0}{load_lower}\of{\gridmeta}
\edef\loadlower{\pgfplotsretval}
\pgfplotstablegetelem{0}{load_upper}\of{\gridmeta}
\edef\loadupper{\pgfplotsretval}
\pgfplotstablegetelem{0}{rho_uniform}\of{\gridmeta}
\edef\rhouniform{\pgfplotsretval}
\pgfplotstablegetelem{0}{rho_specific}\of{\gridmeta}
\edef\rhospecific{\pgfplotsretval}
\pgfplotstablegetelem{0}{q_uniform}\of{\gridmeta}
\edef\quniform{\pgfplotsretval}
\pgfplotstablegetelem{0}{q_specific}\of{\gridmeta}
\edef\qspecific{\pgfplotsretval}
\pgfplotstablegetelem{0}{width_min}\of{\gridmeta}
\edef\widthmin{\pgfplotsretval}
\pgfplotstablegetelem{0}{width_max}\of{\gridmeta}
\edef\widthmax{\pgfplotsretval}
\pgfplotstablegetelem{0}{coverage_target}\of{\gridmeta}
\edef\coveragetarget{\pgfplotsretval}

\newcommand{\drawieeethirtythree}{
    \draw[gridline,line width=0.45pt]
        (axis cs:0,0) -- (axis cs:1.2,0) -- (axis cs:2.4,0)
        -- (axis cs:3.6,0) -- (axis cs:4.8,0) -- (axis cs:6.0,0);
    \draw[gridline,line width=0.45pt]
        (axis cs:6.0,0) -- (axis cs:6.0,-1.5) -- (axis cs:7.2,-1.5)
        -- (axis cs:8.4,-1.5) -- (axis cs:9.6,-1.5)
        -- (axis cs:10.8,-1.5) -- (axis cs:12.0,-1.5)
        -- (axis cs:13.2,-1.5) -- (axis cs:14.4,-1.5)
        -- (axis cs:15.6,-1.5) -- (axis cs:16.8,-1.5)
        -- (axis cs:18.0,-1.5) -- (axis cs:19.2,-1.5);
    \draw[gridline,line width=0.45pt]
        (axis cs:1.2,0) -- (axis cs:1.2,-1.5) -- (axis cs:2.4,-1.5)
        -- (axis cs:3.6,-1.5) -- (axis cs:4.8,-1.5);
    \draw[gridline,line width=0.45pt]
        (axis cs:2.4,0) -- (axis cs:2.4,1.5) -- (axis cs:3.6,1.5)
        -- (axis cs:4.8,1.5);
    \draw[gridline,line width=0.45pt]
        (axis cs:6.0,0) -- (axis cs:6.0,1.5) -- (axis cs:7.2,1.5)
        -- (axis cs:8.4,1.5) -- (axis cs:9.6,1.5)
        -- (axis cs:10.8,1.5) -- (axis cs:12.0,1.5)
        -- (axis cs:13.2,1.5) -- (axis cs:14.4,1.5);
    \draw[gridline,line width=0.35pt]
        (axis cs:13.2,-1.5) -- (axis cs:13.2,-2.05)
        (axis cs:19.2,-1.5) -- (axis cs:19.2,-2.05)
        (axis cs:4.8,-1.5) -- (axis cs:4.8,-2.05)
        (axis cs:4.8,1.5) -- (axis cs:4.8,0.95)
        (axis cs:9.6,1.5) -- (axis cs:9.6,0.95)
        (axis cs:14.4,1.5) -- (axis cs:14.4,0.95);
    % External grid and distribution transformer.
    \node[
        name=externalgrid,
        draw=black,
        line width=0.7pt,
        rectangle,
        pattern=crosshatch,
        pattern color=gray!45,
        minimum width=13pt,
        minimum height=13pt,
        inner sep=0pt
    ] at (axis cs:-2.55,0) {};
    \node[
        name=trafoleft,
        draw=black,
        line width=0.7pt,
        circle,
        fill=none,
        minimum size=8pt,
        inner sep=0pt
    ] at (axis cs:-1.40,0) {};
    \node[
        name=traforight,
        draw=black,
        line width=0.7pt,
        circle,
        fill=none,
        minimum size=8pt,
        inner sep=0pt
    ] at (axis cs:-1.05,0) {};
    \draw[gridline,line width=0.45pt]
        (externalgrid.east) -- (trafoleft.west);
    \draw[gridline,line width=0.45pt]
        (traforight.east) -- (axis cs:0,0);
}

\newcommand{\plotagentdata}[1]{
    % Load agents satisfying the coverage target.
    \addplot[
        only marks,
        scatter,
        scatter src=explicit,
        scatter/use mapped color={draw=black,fill=mapped color},
        mark=*,
        mark size=2.25pt,
        point meta min=\widthmin,
        point meta max=\widthmax,
        restrict expr to domain={\thisrow{plot_class}}{0:0},
        unbounded coords=discard,
    ] table[
        x=plot_x,
        y=plot_y,
        meta=mean_width,
        col sep=comma
    ] {#1};

    % Load agents below the coverage target.
    \addplot[
        only marks,
        scatter,
        scatter src=explicit,
        scatter/use mapped color={
            draw=rwthred100,
            line width=0.9pt,
            fill=mapped color
        },
        mark=*,
        mark size=2.35pt,
        point meta min=\widthmin,
        point meta max=\widthmax,
        restrict expr to domain={\thisrow{plot_class}}{1:1},
        unbounded coords=discard,
    ] table[
        x=plot_x,
        y=plot_y,
        meta=mean_width,
        col sep=comma
    ] {#1};

    % PV agents satisfying the coverage target.
    \addplot[
        only marks,
        mark=pvpanel,
        mark size=3.0pt,
        restrict expr to domain={\thisrow{plot_class}}{2:2},
        unbounded coords=discard,
    ] table[
        x=plot_x,
        y=plot_y,
        col sep=comma
    ] {#1};

    % PV agents below the coverage target.
    \addplot[
        only marks,
        mark=pvpanelalert,
        mark size=3.1pt,
        restrict expr to domain={\thisrow{plot_class}}{3:3},
        unbounded coords=discard,
    ] table[
        x=plot_x,
        y=plot_y,
        col sep=comma
    ] {#1};
}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 2,
        vertical sep=10mm,
    },
    width=0.98\columnwidth,
    height=0.215\columnwidth,
    xmin=-3.1,
    xmax=20.0,
    ymin=-2.35,
    ymax=2.25,
    scale only axis,
    hide axis,
    clip=false,
    filter discard warning=false,
    colormap name=widthmap,
]
\nextgroupplot
\drawieeethirtythree
\plotagentdata{\gridpath/loadwise_rho_grid_uniform.csv}

\nextgroupplot
\drawieeethirtythree
\plotagentdata{\gridpath/loadwise_rho_grid_specific.csv}
\end{groupplot}

\begin{axis}[
    name=widthcolorbar,
    at={($(group c1r2.south)+(0,-7mm)$)},
    anchor=north,
    hide axis,
    scale only axis,
    width=0.72\columnwidth,
    height=0pt,
    point meta min=\widthmin,
    point meta max=\widthmax,
    colormap name=widthmap,
    colorbar horizontal,
    colorbar style={
        width=0.72\columnwidth,
        height=2.4mm,
        xlabel={Mean interval width [p.u.]},
        scaled x ticks=false,
        x tick scale label style={
        at={(axis description cs:1.01,0)},
        anchor=west,
        yshift=1mm,
        },
        xlabel style={font=\scriptsize},
        xticklabel style={
            font=\scriptsize,
            /pgf/number format/fixed,
            /pgf/number format/precision=3,
        },
    },
]
\addplot[draw=none] coordinates {(0,0) (1,1)};
\end{axis}

% Subcaptions underneath the corresponding panels
\node[
    anchor=north,
    font=\footnotesize,
    align=center
] at ([yshift=-2mm]group c1r1.south) {
    (a) Uniform robustness radius, calibrated threshold: 
    {\scriptsize
    $\tau=\pgfmathprintnumber[fixed,precision=2]{\quniform}$}
};

\node[
    anchor=north,
    font=\footnotesize,
    align=center
] at ([yshift=-2mm]group c1r2.south) {
    (b) Loading-specific robustness radius, calibrated threshold:
    {\scriptsize
    $\tau_b=\pgfmathprintnumber[fixed,precision=2]{\qspecific}$}
};

\node[
    circle,
    draw=rwthred100,
    line width=0.9pt,
    minimum size=4.7pt,
    inner sep=0pt
] at ($(group c1r2.south)+(-13mm,-22mm)$) {};
\node[anchor=west,font=\scriptsize]
    at ($(group c1r2.south)+(-12mm,-22mm)$)
    {Coverage below
    $\pgfmathprintnumber[fixed,precision=2]{\coveragetarget}$};
\end{tikzpicture}
\caption{
Robust calibration for load interval
$[\pgfmathprintnumber[precision=3]{\loadlower},
\pgfmathprintnumber[precision=3]{\loadupper}]$ p.u.:
(a) uniform and (b) loading-specific robustness radii.
Bus color denotes mean interval width; red outlines mark trajectory coverage
below the target.
}
\label{fig:loadwise-rho-grid}
\end{figure}


==> figures/agent_location_comparison.tex <==

\providecommand{\locationdatapath}{./agent_location/}
\providecommand{\locationlabelA}{Upstream location}
\providecommand{\locationlabelB}{Central location}
\providecommand{\locationlabelC}{Downstream location}
\providecommand{\locationagentA}{4}
\providecommand{\locationagentB}{0}
\providecommand{\locationagentC}{1}
\providecommand{\locationcoveragefield}{trajectory coverage}
\providecommand{\locationcoveragemin}{0.80}
\providecommand{\locationcoveragetarget}{0.95}

\definecolor{rwthred100}{HTML}{CC071E}
\definecolor{gridline}{HTML}{666666}

\pgfplotsset{
  colormap={coveragemap}{
    rgb255=(255,255,217);
    rgb255=(199,233,180);
    rgb255=(127,205,187);
    rgb255=(65,182,196);
    rgb255=(29,145,192);
    rgb255=(34,94,168);
    rgb255=(12,44,132)
  },
}

\newcommand{\drawieeethirtythree}{
  \draw[gridline,line width=0.45pt]
    (axis cs:0,0)--(axis cs:1.2,0)--(axis cs:2.4,0)
    --(axis cs:3.6,0)--(axis cs:4.8,0)--(axis cs:6.0,0);
  \draw[gridline,line width=0.45pt]
    (axis cs:6.0,0)--(axis cs:6.0,-1.5)--(axis cs:7.2,-1.5)
    --(axis cs:8.4,-1.5)--(axis cs:9.6,-1.5)
    --(axis cs:10.8,-1.5)--(axis cs:12.0,-1.5)
    --(axis cs:13.2,-1.5)--(axis cs:14.4,-1.5)
    --(axis cs:15.6,-1.5)--(axis cs:16.8,-1.5)
    --(axis cs:18.0,-1.5)--(axis cs:19.2,-1.5);
  \draw[gridline,line width=0.45pt]
    (axis cs:1.2,0)--(axis cs:1.2,-1.5)--(axis cs:2.4,-1.5)
    --(axis cs:3.6,-1.5)--(axis cs:4.8,-1.5);
  \draw[gridline,line width=0.45pt]
    (axis cs:2.4,0)--(axis cs:2.4,1.5)--(axis cs:3.6,1.5)
    --(axis cs:4.8,1.5);
  \draw[gridline,line width=0.45pt]
    (axis cs:6.0,0)--(axis cs:6.0,1.5)--(axis cs:7.2,1.5)
    --(axis cs:8.4,1.5)--(axis cs:9.6,1.5)
    --(axis cs:10.8,1.5)--(axis cs:12.0,1.5)
    --(axis cs:13.2,1.5)--(axis cs:14.4,1.5);

  \node[
    draw=black,
    rectangle,
    pattern=crosshatch,
    pattern color=gray!45,
    minimum width=12pt,
    minimum height=12pt,
    inner sep=0pt
  ] (externalgrid) at (axis cs:-2.5,0) {};
  \node[
    draw=black,circle,fill=white,minimum size=7pt,inner sep=0pt
  ] (trafoleft) at (axis cs:-1.4,0) {};
  \node[
    draw=black,circle,fill=white,minimum size=7pt,inner sep=0pt
  ] (traforight) at (axis cs:-1.05,0) {};
  \draw[black,line width=0.7pt]
    (externalgrid.east)--(trafoleft.west)
    (traforight.east)--(axis cs:0,0);
}

\newcommand{\plotlocationagents}[1]{
  % Load agents satisfying the coverage target.
  \addplot[
    only marks,scatter,scatter src=explicit,
    scatter/use mapped color={draw=black,fill=mapped color},
    mark=*,mark size=2.25pt,
    point meta min=\locationcoveragemin,point meta max=1,
    restrict expr to domain={\thisrow{experiment_id}}{#1:#1},
    restrict expr to domain={\thisrow{plot_class}}{0:0},
    unbounded coords=discard
  ] table[
    x=plot_x,y=plot_y,meta=coverage,col sep=comma
  ] {\locationdatapath/agent_location_grid.csv};

  % Load agents below the coverage target.
  \addplot[
    only marks,scatter,scatter src=explicit,
    scatter/use mapped color={
      draw=rwthred100,line width=0.9pt,fill=mapped color
    },
    mark=*,mark size=2.35pt,
    point meta min=\locationcoveragemin,point meta max=1,
    restrict expr to domain={\thisrow{experiment_id}}{#1:#1},
    restrict expr to domain={\thisrow{plot_class}}{1:1},
    unbounded coords=discard
  ] table[
    x=plot_x,y=plot_y,meta=coverage,col sep=comma
  ] {\locationdatapath/agent_location_grid.csv};

  % PV agents satisfying the coverage target.
  \addplot[
    only marks,scatter,scatter src=explicit,
    scatter/use mapped color={draw=black,fill=mapped color},
    mark=square*,mark size=2.25pt,
    point meta min=\locationcoveragemin,point meta max=1,
    restrict expr to domain={\thisrow{experiment_id}}{#1:#1},
    restrict expr to domain={\thisrow{plot_class}}{2:2},
    unbounded coords=discard
  ] table[
    x=plot_x,y=plot_y,meta=coverage,col sep=comma
  ] {\locationdatapath/agent_location_grid.csv};

  % PV agents below the coverage target.
  \addplot[
  only marks,scatter,scatter src=explicit,
    scatter/use mapped color={
      draw=rwthred100,line width=0.9pt,fill=mapped color
    },
    mark=square*,mark size=2.35pt,
    point meta min=\locationcoveragemin,point meta max=1,
    restrict expr to domain={\thisrow{experiment_id}}{#1:#1},
    restrict expr to domain={\thisrow{plot_class}}{3:3},
    unbounded coords=discard
  ] table[
    x=plot_x,y=plot_y,meta=coverage,col sep=comma
  ] {\locationdatapath/agent_location_grid.csv};

  % Diamond ring marking the trained agent's location.
  \addplot[
    only marks,mark=diamond,mark size=4pt,
    draw=black,line width=0.9pt,fill=none,
    restrict expr to domain={\thisrow{experiment_id}}{#1:#1},
    restrict expr to domain={\thisrow{is_location}}{1:1},
    unbounded coords=discard
  ] table[
    x=plot_x,y=plot_y,col sep=comma
  ] {\locationdatapath/agent_location_grid.csv};
}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{groupplot}[
  group style={group size=1 by 3,vertical sep=8mm},
  width=0.98\columnwidth,
  height=0.205\columnwidth,
  xmin=-3.1,xmax=20.0,
  ymin=-2.25,ymax=2.15,
  scale only axis,
  hide axis,
  clip=false,
  filter discard warning=false,
  colormap name=coveragemap,
]

\nextgroupplot[
  title={\textbf{(a) \locationlabelA}\quad
    {\scriptsize trained agent=\locationagentA}},
  title style={
    at={(axis description cs:0,1.10)},
    anchor=west,font=\footnotesize
  },
]
\drawieeethirtythree
\plotlocationagents{0}

\nextgroupplot[
  title={\textbf{(b) \locationlabelB}\quad
    {\scriptsize trained agent=\locationagentB}},
  title style={
    at={(axis description cs:0,1.10)},
    anchor=west,font=\footnotesize
  },
]
\drawieeethirtythree
\plotlocationagents{1}

\nextgroupplot[
  title={\textbf{(c) \locationlabelC}\quad
    {\scriptsize trained agent=\locationagentC}},
  title style={
    at={(axis description cs:0,1.10)},
    anchor=west,font=\footnotesize
  },
]
\drawieeethirtythree
\plotlocationagents{2}

\end{groupplot}
\end{tikzpicture}

\vspace{3mm}
\begin{tikzpicture}
\begin{axis}[
  width=0.98\columnwidth,
  height=0.31\columnwidth,
  xlabel={Agent index},
  ylabel={Trained-agent location},
  xmin=-0.5,xmax=37.5,
  ymin=-0.5,ymax=2.5,
  xtick={0,4,8,12,16,20,24,28,32,37},
  ytick={0,1,2},
  yticklabels={
    \locationlabelC,
    \locationlabelB,
    \locationlabelA
  },
  tick label style={font=\scriptsize},
  label style={font=\small},
  colormap name=coveragemap,
  point meta min=\locationcoveragemin,
  point meta max=1,
  colorbar horizontal,
  colorbar style={
    at={(0.5,-0.42)},
    anchor=north,
    width=0.68\columnwidth,
    height=2.5mm,
    xlabel={Average \locationcoveragefield},
    xlabel style={font=\scriptsize},
    xticklabel style={font=\scriptsize}
  },
]
\addplot[
  matrix plot*,
  mesh/cols=38,
  point meta=explicit
] table[
  x=agent_index,
  y=heatmap_y,
  meta=coverage,
  col sep=comma
] {\locationdatapath/agent_location_heatmap.csv};
\end{axis}
\end{tikzpicture}

\begin{minipage}{0.94\columnwidth}
\scriptsize
\tikz\draw[fill=gray!30] (0,0) circle (2.1pt);
load agent\quad
\tikz\draw[fill=gray!30] (0,0) rectangle (4pt,4pt);
PV agent\quad
\tikz\draw[line width=0.9pt]
  (0,0)--(2pt,2pt)--(4pt,0)--(2pt,-2pt)--cycle;
trained-agent location\quad
\tikz\draw[rwthred100,line width=0.9pt] (0,0) circle (2.1pt);
coverage below \locationcoveragetarget
\end{minipage}

\caption{
Influence of the trained agent's location on robust MA-COPP.
The three IEEE-33 panels show the spatial coverage obtained for each
trained-agent location. Grid color and heatmap cells denote per-agent average
\locationcoveragefield; red outlines identify coverage below the target.
}
\label{fig:robust-agent-location-comparison}
\end{figure}

==> figures/gradual_vs_abrupt/4_coverage_vs_width.tex <==
% Required in the main document preamble:
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}
\providecommand{\datapath}{figures/gradual_vs_abrupt/}

\definecolor{rwthblue100}{HTML}{00549F}
\definecolor{rwthblue50}{HTML}{8EBAE5}
\definecolor{rwthpetrol100}{HTML}{0F4D58}
\definecolor{rwthgray75}{HTML}{7F7F7F}
\definecolor{rwthred100}{HTML}{CC071E}

\pgfplotstableread[col sep=comma]{\datapath/4_coverage_vs_width.csv}\covwidthdata
\pgfplotstablegetelem{0}{coverage_mean}\of{\covwidthdata}
\edef\abruptcoverage{\pgfplotsretval}
\pgfplotstablegetelem{0}{width_mean}\of{\covwidthdata}
\edef\abruptwidth{\pgfplotsretval}
\pgfplotstablegetelem{0}{target_cov}\of{\covwidthdata}
\edef\nominalcoverage{\pgfplotsretval}
\pgfplotstablegetelem{1}{coverage_mean}\of{\covwidthdata}
\edef\gradualcoverage{\pgfplotsretval}
\pgfplotstablegetelem{1}{width_mean}\of{\covwidthdata}
\edef\gradualwidth{\pgfplotsretval}
\pgfmathsetmacro{\widthymax}{1.18*max(\abruptwidth,\gradualwidth)}

\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    width=0.84\columnwidth,
    height=0.58\columnwidth,
    xlabel={Target coverage},
    ylabel={Mean interval width (p.u.)},
    xmin=0.94,
    xmax=1.003,
    ymin=0,
    ymax=\widthymax,
    xtick={0.95,0.97,0.99,1.00},
    ytick={0,0.02,0.04,0.06},
    scaled y ticks=false,
    y tick label style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2,
        font=\footnotesize,
    },
    x tick label style={font=\footnotesize},
    label style={font=\footnotesize},
    axis line style={black!65},
    tick style={black!65},
    clip=false,
]
\addplot[
    only marks,
    mark=*,
    mark size=4pt,
    draw=black,
    fill=rwthred100,
] coordinates {(\abruptcoverage,\abruptwidth)};

\addplot[
    only marks,
    mark=*,
    mark size=4pt,
    draw=black,
    fill=rwthpetrol100,
] coordinates {(\gradualcoverage,\gradualwidth)};

\addplot[sharp plot, no marks, rwthblue100, dashed, thick]
    coordinates {(\nominalcoverage,0) (\nominalcoverage,\widthymax)};

\node[font=\scriptsize, anchor=south east, xshift=-2pt, yshift=2pt]
    at (axis cs:\abruptcoverage,\abruptwidth) {Abrupt};
\node[font=\scriptsize, anchor=north east, xshift=-2pt, yshift=-2pt]
    at (axis cs:\gradualcoverage,\gradualwidth) {Gradual};
\end{axis}
\end{tikzpicture}
\caption{Coverage--width trade-off on the shared 3RL target. The dashed line marks nominal coverage; lower interval width is preferable at valid coverage.}
\label{fig:coverage_vs_width}
\end{figure}


==> figures/results_ieee141/robust_rho_plot.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{groupplot}[
            group style={
                group size=2 by 1,
                horizontal sep=1.2cm
            },
            width=4.5cm,
            height=4.0cm,
            xlabel={$\rho$},
            grid=both,
            grid style={line width=.1pt, draw=rwthgray75!30},
            tick label style={font=\footnotesize},
            label style={font=\footnotesize}
        ]
            % --- LEFT PLOT: Coverage ---
            \nextgroupplot[
                ylabel={coverage},
                extra y ticks={0.95},
                extra y tick labels={},
                extra y tick style={
                    grid=major,
                    grid style={rwthred100, dashed, line width=1.0pt}
                }
            ]
            \addplot[color=rwthblue100, mark=*, mark size=1.2pt, thick]
                table [x=rho, y=coverage, col sep=comma]
                {figures/results_ieee141/robust_sweep_chi2_max_uniform.csv};

            % --- RIGHT PLOT: Width ---
            \nextgroupplot[
                ylabel={avg. region width [p.u.]}
            ]
            \addplot[color=rwthblue100, mark=*, mark size=1.2pt, thick]
                table [x=rho, y=width, col sep=comma]
                {figures/results_ieee141/robust_sweep_chi2_max_uniform.csv};

        \end{groupplot}

        % Subfigure labels underneath each plot
        \node[font=\footnotesize, anchor=north]
            at ($(group c1r1.south) + (0,-0.75cm)$)
            {(a) Empirical coverage};

        \node[font=\footnotesize, anchor=north]
            at ($(group c2r1.south) + (0,-0.75cm)$)
            {(b) Average width};

    \end{tikzpicture}
    \caption{Robustness-radius sweep analysis for the IEEE 141-bus grid.}
    \label{fig:ieee141-rho-sweep}
\end{figure}

==> figures/results_ieee33/robust_rho_plot_33.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{groupplot}[
            group style={
                group size=2 by 1,
                horizontal sep=1.2cm
            },
            width=4.5cm, % Kept small to fit a two-column width comfortably
            height=4.0cm,
            xlabel={$\rho$},
            grid=both,
            grid style={line width=.1pt, draw=rwthgray75!30},
            tick label style={font=\tiny},
            label style={font=\scriptsize}
        ]
            % --- LEFT PLOT: Coverage ---
            \nextgroupplot[
                ylabel={coverage},
                % This adds an extra tick line cleanly at 0.95 without using dynamic coordinate calculation
                extra y ticks={0.95},
                extra y tick labels={}, % Keeps it from cluttering the axis labels
                extra y tick style={grid=major, grid style={rwthred100, dashed, line width=1.0pt}}
            ]
            \addplot[color=rwthblue100, mark=*, mark size=1.2pt, thick] 
                table [x=rho, y=coverage, col sep=comma] {figures/results_ieee33/robust_sweep_chi2_max_uniform.csv};

            % --- RIGHT PLOT: Width ---
            \nextgroupplot[ylabel={avg region width [p.u.]}]
            \addplot[color=rwthblue100, mark=*, mark size=1.2pt, thick] 
                table [x=rho, y=width, col sep=comma] {figures/results_ieee33/robust_sweep_chi2_max_uniform.csv};
                
        \end{groupplot}
    \end{tikzpicture}
    \label{fig:IEEE33_robustness_radius}
    \caption{Robustness radius sweep analysis for the IEEE33 grid.}
\end{figure}

==> figures/results_ieee33/voltage_plot_33.tex <==
\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \begin{axis}[
            width=8cm, 
            height=5cm,
            xlabel={Time step},
            ylabel={Voltage [p.u.]},
            label style={font=\small},
            tick label style={font=\small},
            grid=both,
            grid style={line width=.1pt, draw=rwthgray75!30},
            legend style={at={(0.02,0.02)}, anchor=south west, font=\tiny, draw=none, fill=white, fill opacity=0.8},
            unbounded coords=jump, 
            xmin=0,
            % Ensure limits are strictly set/enforced for layering
            set layers=standard 
        ]
            
            % 1. Conformal Region (Interval Fill)
            \addplot[name path=A, transparent, forget plot] table [x=time, y=lower_interval, col sep=comma] {figures/results_ieee33/voltage_plot_data_ieee33.csv};
            \addplot[name path=B, transparent, forget plot] table [x=time, y=upper_interval, col sep=comma] {figures/results_ieee33/voltage_plot_data_ieee33.csv};
            \addplot[rwthblue50!50, opacity=0.5] fill between[of=A and B];
            \addlegendentry{Conformal Region}

            % 2. Historical Line (Prefix)
            \addplot[color=rwthpetrol100, line width=1.8pt, no marks] table [x=time, y=historical, col sep=comma] {figures/results_ieee33/voltage_plot_data_ieee33.csv};
            \addlegendentry{Historical}

            % 3. Real Future Line (Suffix)
            \addplot[color=rwthred100, line width=1.0pt, no marks] table [x=time, y=real_future, col sep=comma] {figures/results_ieee33/voltage_plot_data_ieee33.csv};
            \addlegendentry{Real Future}

            % 4. Prediction Line (Suffix)
            % Added 'dash pattern' explicitly to keep it looking crisp at 8cm width
            \addplot[color=rwthblue100, line width=1.4pt, dash pattern=on 3pt off 2pt, no marks] table [x=time, y=prediction, col sep=comma] {figures/results_ieee33/voltage_plot_data_ieee33.csv};
            \addlegendentry{Prediction}

            % 5. Vertical Split Line (Moved to the end)
            % Drawing this last ensures it reads the finalized ymin/ymax and sits ON TOP of the fill region
            \draw[draw=rwthgray75, dash pattern=on 1pt off 1.5pt, line width=1.2pt] 
                (axis cs:20, \pgfkeysvalueof{/pgfplots/ymin}) -- (axis cs:20, \pgfkeysvalueof{/pgfplots/ymax});

        \end{axis}
    \end{tikzpicture}
        \label{fig:IEEE33_cp_interval}
    \caption{Voltage prediction with conformal intervals for one agent in the IEEE33 grid.}
\end{figure}

==> intro_clean.tex <==

\section{Introduction}

Power systems are undergoing a structural transition from relatively predictable, centrally managed infrastructures to more decentralized, power-electronics-dominated, and data-rich grids. This change is especially visible at the distribution level, where numerous inverter-interfaced distributed energy resources (DERs), flexible loads, and heterogeneous control devices operate as independent decision-making components, forming a complex \textit{multi-agent} environment that shapes real-time operations. One of the growing challenges in managing active grids is maintaining bus voltages within permissible safe limits, as the increasing penetration of intermittent renewable generation can lead to severe voltage fluctuations and oscillatory behavior \cite{MURRAY2021111100}. Conversely, smart inverters can provide fast, continuous reactive power support, enabling adaptive voltage regulation \cite{CUI2022108609}. To automate this Volt-Var control problem, various control \textit{policies}, or automated decision-making rules, have been proposed, ranging from simple rule-based local droop schemes to advanced learning-based methods like reinforcement learning \cite{GLA19,ZHA21,Wang2020SafeOffPolicy,Gao2021ConsensusMARL,Kabir2023TwoTimescaleVVC,Wang2021MARLVoltage}. However, because these autonomous agents often act based on local data, they may fail to guarantee grid-wide safe voltage regulation due to the lack of coordination \cite{Saverio2019} or the uninterpretable "black box" nature of deep learning schemes. Therefore, an important open question is whether such distributed control approaches can be validated for safe closed-loop operation when interacting dynamically with the physical distribution grid and adjacent control actuators.

Assuring the safe deployment of new controllers involves two complementary paradigms: validation, which evaluates performance using physical simulations or empirical tests, and verification, which provides analytical safety proofs. In distribution systems, both paths are exceptionally difficult because grid operators do not possess a high-fidelity model of the real-grid. Instead, grid models are affected by limited observability, data-quality issues, and imperfect topology knowledge \cite{Geth2023DSSEPractical,Parlaktuna2024TopologyError}, alongside uncertainties from renewable injections, load behavior, measurement noise, and unmodeled dynamics \cite{Wang2025UncertaintyReview}. Traditional validation tools, such as scenario simulation and hardware-in-the-loop testing \cite{Wang2019PHIL,OTT18,PAS24}, rely on these imperfect models; however, because a real distribution grid contains a vast density of heterogeneous components, establishing a perfect simulation oracle is practically impossible. Consequently, validation is forced to rely on simplified assumptions, evaluates only finitely many scenarios, and cannot eliminate simulation-to-reality mismatches or test directly against the true physical grid. Furthermore, because available historical data are typically generated under previously deployed controllers, they do not directly validate a new candidate configuration, leaving grid operators with a critical, system-level deployment question:
\emph{If one or more inverter controllers are modified, will all voltages remain within their admissible limits over the considered future horizon?}

Analytical verification workflows share these identical modeling bottlenecks. On one hand, formal verification, reachability analysis, and certificate-based methods provide strong deterministic guarantees, but they require accurate models, tractable mathematical abstractions, and substantial computational cost \cite{ALT14,AlthoffKrogh2014DAE,Tran2022VerificationLECPS,Everett2021NNVerification,Kochdumper2023OpenClosedLoop,Dawson2023LearnedCertificates}. On the other hand, safe reinforcement-learning techniques embed safety layers for constraint satisfaction directly into controller design to minimize baseline operational risks, though often at the cost of more restrictive exploration, constraint tightening, or degraded performance \cite{Wang2020SafeOffPolicy,Gao2022ModelAugmentedSafeRL,Nguyen2022OnlineSafeDRL}. Because both validation and verification workflows ultimately rely on simplified modeling assumptions or assume high-fidelity models, neither paradigm in isolation can eliminate simulation-to-reality gaps or guarantee safety under complex multi-agent interactions and deployment-level distribution shifts. 

Statistical methods provide another direction for handling system uncertainty. Chance-constrained optimization-based voltage-control schemes typically require an assumed uncertainty distribution \cite{Li2019, Mieth2018}, while Gaussian-process-based uncertainty quantification often relies on Gaussian assumptions and does not generally provide finite-sample coverage guarantees for the resulting intervals \cite{pareek2025learningpowerflowconfidence,MOLLAALI2025107809}. Conformal Prediction (CP) offers a complementary data-driven approach: instead of specifying the full uncertainty distribution, it uses past prediction errors to calibrate uncertainty sets with distribution-free coverage guarantees. CP has recently been applied in power and energy settings, including PV forecasting and stochastic decision-making \cite{REN24,Renkema2024PVForecast}.

The problem at hand here is not only to forecast future voltages, but to support pre-deployment safety assessment of a candidate controller. The available model or simulator provides a predicted future voltage trajectory for the tested operating scenario. This trajectory is treated as a reference prediction, not as an exact description of the future grid behavior. We therefore use historical discrepancies between predicted and realized voltage trajectories to construct an uncertainty band around the predicted trajectory, and we check safety using this band rather than the prediction alone.

The main additional challenge here is controller replacement. Historical data are usually collected under a baseline controller, whereas deployment may use a new candidate controller at one or more buses. This control rule change can alter reactive-power commands, power flows, voltage profiles, and the simulation-to-reality voltage-error distribution. Standard CP relies on calibration and deployment cases being sufficiently aligned and can lose validity when this alignment is broken \cite{TIB20,BAR23}. Existing off-policy and multi-agent conformal prediction methods address related controller-switching questions \cite{TAU22,KUI24}, but they are not designed as system-level voltage-safety layers for distribution grids and can become overly conservative when baseline and candidate controllers differ substantially. Robust validation and robust conformal methods therefore provide a natural way to protect calibrated sets against bounded changes in the error distribution \cite{CAU24,AOL25}.


To address this problem, the framework proposed in this paper is designed to operate as an overarching statistical screening layer that complements all of these methods; it utilizes the nominal predictor as the reference baseline, treating any underlying control synthesis, simulation model, or internal verification pipeline as a black box to provide a final, distribution-free statistical safety check before field activation.

The proposed method, called the \emph{Distributionally Robust Conformal Safety Screening} (DR-CSS), combines these ideas in the distribution power-system setting. Conventional scenario simulation checks only whether one nominal simulated voltage trajectory violates the limits. DR-CSS instead builds a calibrated voltage uncertainty band around that trajectory, widens the band to account for controller-induced changes in simulation-to-reality error behavior, and returns an accept/warning decision for the tested operating scenario. The scenario is accepted only if the full robust band remains inside the admissible voltage limits over the look-ahead horizon. A detailed positioning of DR-CSS relative to related assurance approaches is provided in Appendix~\ref{app:positioning}.

The broader deployment message is not that learning-based voltage control should be rejected, but that it should be introduced conservatively. When a candidate inverter policy cannot yet be fully trusted, it is operationally reasonable to activate it gradually, apply it only to part of the distribution network or a subset of devices, collect new closed-loop data, and re-evaluate safety before broader rollout. Such staged deployment reduces the magnitude of controller-induced error changes, makes failures easier to localize, and matches the validation logic developed in this paper.

The main contributions of this paper are as follows:
\begin{itemize}
    \item We propose DR-CSS, a general distributionally robust conformal safety-screening methodology for closed-loop controller deployment under simulation-to-reality error and controller-induced distribution shift.

    \item We specialize DR-CSS to active distribution-grid voltage control and derive a trajectory-level voltage safety score that checks all buses and all future time steps.

    \item We validate the method on IEEE 33-bus and IEEE 141-bus feeders, showing near-target coverage, tighter bands than weighted off-policy conformal baselines, and reduced conservativeness through context-aware calibration and gradual deployment.
\end{itemize}

The remainder of the paper is organized as follows. Section~II formulates the voltage-control and deployment-assessment problem. Section~III presents DR-CSS. Section~IV reports the numerical results. Section~V concludes the paper.

